Learning task structure via sparsity grouped multitask learning

Sparse mapping has been a key methodology in many high-dimensional scientific problems. When multiple tasks share the set of relevant features, learning them jointly in a group drastically improves the quality of relevant feature selection. However, in practice this technique is used limitedly since such grouping information is usually hidden. In this paper, our goal is to recover the group structure on the sparsity patterns and leverage that information in the sparse learning. Toward this, we formulate a joint optimization problem in the task parameter and the group membership, by constructing an appropriate regularizer to encourage sparse learning as well as correct recovery of task groups. We further demonstrate that our proposed method recovers groups and the sparsity patterns in the task parameters accurately by extensive experiments.

==> complexity_original.tex <==
\section{Sample Complexity}

\newcommand{\Fcal}{\ensuremath{\mathcal{F}}}
\newcommand{\balpha}{\ensuremath{\bm \alpha}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}

It is natural to ask whether enforcing the shared sparsity structure,
when groups are unknown leads to any efficiency in the number of
samples required for learning. We now examine this question from two
viewpoints. Let us begin with an overly simplistic setup, where the
structural assumptions which motivate our
objective~\eqref{EqnBaseline} hold exactly. That is, consider that the
parameters form $N$ groups, with the weights in each group taking
non-zero values only on a common subset of features of size at most
$s$. Let us also consider the simplest inefficient method in this
case, a generalization of subset selection for Lasso which searches
over all subsets of size $s$. It picks one subset $S_G$ for each group
$G$ and then estimates the weights independently for each task in
group $G$, allowing non-zero values only on $S_G$. Using a simple
parameter counting argument, we expect this computationally efficient,
but statistically sound method to find the right support sets, as well
as good parameter values once the number of samples exceeds $O(N
s\log J + ms)$. This follows since the first term captures the
complexity of selecting the right subset out of $\choose{J}{s}$
possibilities for each group, followed by the independent parameter
estimation of $s$ weights for each task. We contrast this with the
number of samples which would be required for a similarly inefficient
approach to solve each task independently, only leveraging the
sparsity of the task. In this case, we are solving essentially $s$
independent Lasso problems, meaning we will require $O(ms\log J)$
samples to find the good parameter estimates.\footnote{Alternatively,
  one can compare $O(s\log J)$ samples per task in the na\"ive
  approach, with $O(s + N s\log J/m)$ using the group sparsity
  structure.} We note that exploiting group structure removes any
direct interaction between the number of tasks $m$ and the ambient
dimension $J$, which can be particularly beneficial when the number of
groups $N \ll m$. 

Alternatively, one could consider the entire
collection of tasks as one group, and use $\|\cdot\|_{1,2}$
regularization on the weight matrix to enforce shared sparsity
structure. However, we now need to find a feature subset of size
$sN$, since that is the size of the shared support across all
tasks. While this yields the correct complexity $O(N s\log J)$ in
searching for the union of the supports, the subsequent weight
estimation unavoidably scales as $O(msN)$, since that is the number
of non-zero weights we are forced to estimate per task instead of
$O(s)$ weights for our approach. In summary, this reasoning, albeit a
bit crude, motivates why learning the task structure jointly with the
weights can be beneficial when our modeling assumption is a good fit,
and how it can gain substantially over natural baselines on the two
extreme ends of our spectrum.

While the above reasoning serves as a good motivation, it does not
capture the actual sample complexity of our method well, which does
not perform inefficient search over subsets, and uses the regularized
formulation of Equation~\ref{EqnGrpLearn3} instead. It is well-known
in the statistical learning theory literature that the generalization
error of regularized objectives can be understood through the
Rademacher complexity of the set of functions where the regularizer
takes small values (see e.g.~\citet{Bartlett2002}). With this in mind,
we now provide a bound on the Rademacher complexity of the set of
$(\U_1, \ldots, \U_{N}, \W)$ tuples (denoted concisely as
$(\U_{1:N}, \W)$) where the regularizer in
Equation~\ref{EqnGrpLearn3} is bounded. Formally, let us define a
class of matrix tuples indexed by a vector $\balpha \in \reals^{N}$
as:
\begin{align}
  \Fcal_{\balpha}(\U_{1:N}, \W) &= \{(\U_{1:N}, \W)~|~
  \|\sqrt{\U_g}\W\|_{1,2} \leq \alpha_g,\nonumber\\ &\sum_{g \in \G} \U_g =
  \I^{m\times m}, [\U_g]_{jk} \in [0,1]\}.
\label{EqnRadClass}
\end{align}
%
We suppress the subscript $1:N$ in the $\U$ matrices in the sequel,
since it is fixed in the context. Then we will study the Rademacher
complexity of the class of linear predictors defined via the $\W$
matrices, that is
\begin{equation}
R_n(\Fcal_{\balpha}) = \frac{1}{nm} \EE_\sigma\left[\sup_{(\U, \W) \in
    \Fcal} \sum_{t=1}^m\sum_{i=1}^n \sigma_{t,i} w_t^\top x_{t,i}
  \right],
\label{EqnRadDef}
\end{equation}
%
where $\sigma_{t,i}$ are i.i.d. $\pm 1$-valued random variables with
mean 0, and we assume that we have $n$ samples $(x_{t,1}, \ldots,
x_{t,n})$ for each task $t$. Note that while we study the complexity
of linear functions, this is directly influences the generalization
error when using Lispchitz loss functions on the prediction of such a
linear function using standard contraction arguments (see e.g. result
4, Theorem 12 of~\citet{Bartlett2002}). We now present a bound on this
Rademacher complexity. 

\begin{theorem}
  Assume that all data points $x$ satisfy $\|x\|_\infty \leq X$. Then
  the Rademacher complexity of the class of
  matrices~\eqref{EqnRadClass} admits the bound 
  \begin{align*}
    R_n(\Fcal_{\balpha}) &\leq 2X\sqrt{\frac{\log 2nJ}{n}}\, \frac{\sum_{g \in
        \G} \alpha_g}{m}.
  \end{align*}
\end{theorem}

The bound is always better than independent Lasso for each task, since
$\alpha_g \leq \|\W\sqrt{\U_g}\|_{1,1}$, which recovers the Lasso
bound. In general, if we have a small number of groups relative to the
number of tasks, with a significant overlap in the sparsity structures
within each group, we expect an improvement of $g/m$ in the sample
complexity over not utilizing the group structure. The proof of this
theorem is presented in the appendix.


==> complexity_proof.tex <==


\onecolumn
\begin{proof}
  The proof follows standard arguments for bounding the Rademacher
  complexity of norm balls in linear prediction, along with some
  modifications to account for the group structure of our problem. We
  suppress the subscript $\balpha$ on $\Fcal$ and observe that
  \begin{align*}
    R_n(\Fcal) &= \frac{1}{nm} \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal}
  \sum_{t=1}^m\sum_{i=1}^n \sigma_{t,i} w_t^\top x_{t,i} \right]\\
    &= \frac{1}{nm} \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal}
  \sum_{t=1}^mw_t^\top \left(\sum_{i=1}^n \sigma_{t,i}
  x_{t,i}\right)\right]. 
  \end{align*}
  Let us define the shorthand $\xi_t = \sum_{i=1}^n \sigma_{t,i}
  x_{t,i}/n$. Since $\sum_{g\in \G} [\U_g]_{t,t} = 1$ for all tasks
  $t$, we can further rewrite the above as

  \begin{align*}
    R_n(\Fcal) &= \frac{1}{m} \EE_\sigma\left[\sup_{(\U, \W) \in
        \Fcal} \left(\sum_{g \in \G} [\U_g]_{t,t}
      \right)\sum_{t=1}^mw_t^\top \xi_t\right]\\
    &= \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal} \frac{1}{m} \sum_{g
        \in \G} \sum_{t=1}^m [\U_g]_{t,t}w_t^\top \xi_t \right]\\
    &= \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal} \frac{1}{m} \sum_{g
        \in \G} \text{Tr}(\U_g\W^\top\xi) \right]\\
    &= \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal} \frac{1}{m} \sum_{g
        \in \G} \text{Tr}(\sqrt{\U_g}\W^\top\xi\sqrt{\U_g}) \right]\\
    &\leq \EE_\sigma\left[\sup_{(\U, \W) \in \Fcal} \frac{1}{m} \sum_{g
        \in \G} \|\xi\sqrt{U_g}\|_{\infty,
        2}\|\W\sqrt{\U_g}\|_{1,2}\right]\\
    &\leq \frac{1}{m} \EE_\sigma \sum_{g \in \G}
      \|\xi\sqrt{\U_g}\|_{\infty, 2} \alpha_g, 
  \end{align*}
  %
  where the last equality uses the matrix $\xi \in \reals^{J\times m}$
  to collect the $\xi_t$ vectors for each task as column
  vectors, and the final inequality uses H\"older's inequality for the
  matrix inner product defined as $\text{Tr}(A^\top B)$ and with the
  dual norm pair $\|\cdot\|_{1,2}$ and $\|\cdot\|_{\infty,2}$.

%% Since $[\U_g]_{j,k} \in [0,1]$ and norms are absolutely
  %% symmetric, we further obtain 
  
  %% \[
  %% \|\W\U_g\|_{1,2} \leq \||\W|\U_g\|_{1,2} \leq
  %% \||\W|\sqrt{\U_g}\|_{1,2} = \|\W\sqrt{\U_g}\|_{1,2} \leq \alpha_g. 
  %% \]
  
  %% Hence we can further simplify as
  %%
  %% \[
  %% R_n(\Fcal) &\leq \frac{1}{m} \EE_\sigma \sum_{g \in \G}
  %% \|\xi\|_{\infty, 2} \alpha_g.
  %% \]

  Hence, it remains to bound
  $\EE_\sigma\|\sqrt{U_g}\xi^\top\|_{\infty, 2}$ to complete our
  proof. By definition of the norms, we and recalling the definition
  of $\xi$ we have
  \[
  \EE_\sigma \|\sqrt{U_g}\xi^\top\|_{\infty, 2} = \EE_\sigma
  \max_{j=1,\ldots,J}\sqrt{\sum_{t=1}^m [\U_g]_{t,t} \left(\frac{1}{n}
    \sum_{i=1}^n \sigma_{t,i} x_{t,i}(j) \right)^2}. 
  \]
  % 
  Let us consider the random variable $\xi_t(j) = \frac{1}{n}
  \sum_{i=1}^n \sigma_{t,i} x_{t,i}(j)$ for any task $t$. For now, let
  us hold the $x_{t,i}(j)$ as fixed, and analyze the random variables
  $\sigma_{t,i}$ which are i.i.d. and zero mean. So by Hoeffding's
  inequality and a union bound, we see that with probability at least
  $1 - \delta$ (over the draw of the $\sigma$'s)
  \[
  \max_{j=1,\ldots, J} \left|\frac{1}{n}
  \sum_{i=1}^n \sigma_{t,i} x_{t,i}(j)\right| \leq \frac{1}{n}
  \sqrt{\frac{\sum_{i=1}^n x_{t,i}(j)^2}{2}\log\frac{2J}{\delta}}. 
  \]
  %
  Since $x_{t,i}(j) \leq X$ by assumption, with probability at least
  $1/n$, we have
  \[
  \max_{j=1,\ldots, J} \left|\frac{1}{n} \sum_{i=1}^n \sigma_{t,i}
  x_{t,i}(j)\right| \leq \sqrt{\frac{X^2}{2n}\log 2nJ}.
  \]
  
  Using this bound, and that $\xi_t(j) \leq X$ always, we further
  obtain that
  \begin{align*}
  \EE_\sigma \|\sqrt{U_g}\xi^\top\|_{\infty, 2} &\leq
  \sqrt{\sum_{t=1}^m [\U_g]_{t,t} \left(\frac{X^2}{2n}\log 2nJ +
    \frac{X^2}{n}\right)}
  \leq 2X\sqrt{\frac{\log 2nJ}{n}}.
  \end{align*}
  %
  Collecting terms, we finally have the desired upper bound on the
  Rademacher complexity since 

  \begin{align*}
    R_n(\Fcal) &\leq \frac{1}{m} \EE_\sigma \sum_{g \in \G}
    \|\xi\sqrt{U_g}\|_{\infty, 2} \alpha_g\\
    &\leq \frac{1}{m} \sum_{g \in \G} \alpha_g  \,2X\sqrt{\frac{\log
        2nJ}{n}}.
  \end{align*}
\end{proof}


==> relatedwork.tex <==
Additional relevant work to model task relatedness include the work of~\cite{EvPon2007} which considers that all task share the same set of relevant features thereby grouping all the tasks together.  Another line of work  consists in assuming that the relationships among tasks are governed by a latent feature representation~\cite{Caruana1997}. Another pertinent approach which assumes latent basis tasks is that in~\cite{Kumar2012}  which considers learning potentially overlapping task groups  assuming that task parameters within a group lie in a low dimensional subspace.




